Observations on Porting In-memory KV stores to Persistent Memory

Systems that require high-throughput and fault tolerance, such as key-value stores and databases, are looking to persistent memory to combine the performance of in-memory systems with the data-consistent fault-tolerance of nonvolatile stores. Persistent memory devices provide fast bytea-ddressable access to non-volatile memory. We analyze the design space when integrating persistent memory into in-memory key value stores and quantify performance tradeoffs between throughput, latency, and and recovery time. Previous works have explored many design choices, but did not quantify the tradeoffs. We implement persistent memory support in Redis and Memcached, adapting the data structures of each to work in two modes: (1) with all data in persistent memory and (2) a hybrid mode that uses persistent memory for key/value data and non-volatile memory for indexing and metadata. Our experience reveals three actionable design principles that hold in Redis and Memcached, despite their very different implementations. We conclude that the hybrid design increases throughput and decreases latency at a minor cost in recovery time and code complexity

==> section/discuss.tex <==
\section{Discussions}
Through the implementation of Hybrid and Fully Persistent versions of Redis and
Memcached, we were able to formulate four actionable design principles that
developers should follow when porting volatile key/value stores to persistent
memory. These principles include keeping in mind that there is a direct
tradeoff between data consistency and performance, using a fully featured
persistent library for Hybrid Designs, using a hybrid schema is preferable, and
data should be allocated in large chunks. 

%For developers to fully consider all these factors is nontrivial as they have
%interesting tradeoffs. As a result, we framed our key findings with some
%guiding principles to use when porting storage systems to Persistent Memory.

\begin{enumerate}[
leftmargin=0pt, itemindent=20pt,
labelwidth=15pt, labelsep=5pt, listparindent=0.7cm,
align=left]
	\item Direct tradeoff between data consistency and performance.  

    For Base Redis, this relationship is easily seen as the frequency you choose to
    snapshot your memory state into disk is directly related to how poorly your
    system performs. If you snapshot to disk frequently, you experience more
    frequent drops in throughput, with these drops in throughput leading to
    very poor performance as seen in Figure \ref{fig:snapshot}. With this poor
    performance for persistence, ensuring snapshots after every key value
    modification is unrealistic leading to poor data consistency as a direct
    result.

    Since the fully persistent and hybrid designs work with persistent data, they
    both have the same interaction with data consistency and performance. The
    amount of data loss that Persistent KV Stores see is dependent on the
    granularity of your transaction size. You can have a transaction for every
    key-value pair you insert, but since you have multiple transactions the
    cost of flushing and committing frequently will negatively effect
    performance. If you have a more coarse-grained transaction with one
    transaction covering multiple key-value modifications at once, performance
    will slightly increase at the cost of transaction rollback in the case of
    system failure during a transaction. However, the negative impact of
    transactions on performance is much lighter than Base Redis' disk-based
    accesses, making transactions for every key-value pair more feasible than
    snapshots for every key-value pair. The main difference between the Hybrid
    Design and Fully Persistent Design here is that the Fully Persistent Design
    has to account for the data consistency of the Persistent Hashtable as well
    as the key-value pairs. This leads to the Fully Persistent Design having to
    either use more transactions or larger-scale transactions and subsequently
    suffer drops in throughput or data consistency.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=3.2in]{transactions.png}
%   \caption{Performance Characteristics of Base Redis Snapshotting vs Persistent Memory Transactions where Data Loss is the same for both consistency mechanisms}
%   \label{fig:performance}
% \end{figure}

  \item Full featured persistent memory libraries ease developement and lead to
    simple implementations for the Hybrid Design.

    In order to have a method of reading persistent data upon restart, developers
    either have to maintain their own auxiliary persistent data structure or
    rely on their persistent memory library to recollect data. While some
    libraries might store persistent data contiguously and make any reads from
    persistent files inconsequential, other libraries such as pmdk may require
    one to make some modifications to keep track of persistent data addresses.
    Without relying on a persistent memory library, developers will have to
    manually create their own persistent data storage method or structure.
    These findings are directly taken from our observations when we  maintained
    our own auxiliary data structure for Hybrid Redis. We found that creating
    our own data structure was not only a significant development effort to
    maintain but was also difficult to keep efficient.  As a result, we
    switched to using the pmdk allocator linked list for Hybrid Redis. On the
    other hand, pmdk's allocator linked list was inefficiently constructed so
    developers have to keep in mind that they may be limited with regards to
    this aspect when choosing the Hybrid Design.

  \item A hybrid design is preferable. The improved recovery performance of a
    fully-persistent implementation is not worth the performance overhead on
    every I/O. \bch{Do we keep this arguement, get rid of it or remodel the
    argument to say hybrid design is preferable for those who prioritize
    performance and fully persistent design is ideal for those who want an
    efficient recovery time?}

    The hybrid design pays a small recovery overhead to realize far less
    performance overhead than the Fully Persistent design, which we deem to be
    preferable. Although persistent indexing structures can bring near nonexistent
    recovery time, this is not a compelling enough reason to choose the Fully
    Persistent Design for several reasons. First, for many modern applications,
    ensuring quick turnaround time and operational performance is of utmost
    importance to users. Especially for distributed database and KV Store
    applications that receive a large amount of requests and accesses from clients.
    Although recovery performance is also important, it generally remains as an
    auxiliary thought to the operational throughput. 
    %Even with persistent memory, you still need to design hybrid data structures
    %that separate persistent data from volatile indexing as one should be happy to
    %pay a small recovery overhead to realize runtime benefit and performance. 
    Second, the hybrid design still offers a relatively respectable recovery time
    that is comparable to the Base Redis recovery time. As long as recovery
    performance is not increased to an unacceptable level by the persistent memory
    library or persistent storage structure one chooses, the Hybrid Design can
    still remain usable.  Finally, the fully persistent recovery performance is
    only efficient when not using a transaction. When using a transaction to ensure
    data consistency during recovery, the performance drastically decreases. One
    could combat this by making more modifications to your data structures to avoid
    any persistent memory writes but this requires significant development efforts.
    This could also be fixed by not using a transaction and not issuing any data
    consistency measures during recovery. However, this method leads to potential
    issues when a system failure occurs during recovery, which is more likely as
    your recovery time will scale up with large-scale databases.

    \bch{New Argument could be: The hybrid design realizes far less performance
    overhead than the Fully Persistent Design while also being much more stable.
    For many modern applications, ensuring quick turnaround time and operational
    performance is of utmost importance to users. Especially for distributed
    database and KV Store applications that receive a large amount of requests and
    accesses from clients. Although recovery performance is also important, it can
    remain as an auxiliary thought to the operational throughput and tail latency
    for some users. On the other hand, fully persistent indexing structures can
    bring near nonexistent recovery time at the cost of performance drops. For many
    large-scale databases or applications that work with a surplus of data, having
    quick recovery time can be crucial in order to ensure that users aren't waiting
    for long periods of time after any crashes.}

\item  Comparison of Redis vs Memcached. Data must be allocated in large chunks
  to amortize the increased latency of persistent memory.

  When performing allocations in persistent memory, it is much more efficient to
  have preemptive large chunk allocations inorder to amortize the increased
  latency of persistent memory. One of the major differences between Redis and
  Memcached that heavily influenced the porting procedure to persistent memory
  was the differing allocation schemes. Just as a designer should aim to reduce
  the number of writes in persistent memory, they should also aim to reduce the
  number of allocations in persistent memory due to its high cost and performance
  inefficiency. Having a per-key/value pair allocation schema in a volatile key
  value store is still reasonable as the performance costs of volatile allocation
  are negligible and the complexity of managing larger allocations can be
  cumbersome. However, persistent allocations require writes to persistent memory
  which incurs a much larger performance cost than volatile writes.  The major
  design choice we observed with Redis' per key value allocation schema and
  Memcached's slab-based allocation schema was that allocating persistent data in
  larger chunks greatly helps amortize the costs of allocation. This way,
  operational performance is maintained with allocations only being necessary
  when allocating a new slab.

\end{enumerate}

%\subsection{New Key Points}
%\begin{enumerate} \item Even with Persistent memory, you still need to design
%hybrid data structures that separate persistent data from volatile indexing ->
%happy to pay a small recovery overhead to realize runtime benefit and
%performance.  (Similar to Point 3 of old key points, combine here)

%	\item  Comparison of Redis vs Memcached. Increased latency of persistent
%	memory requires you to allocate persistent data in large chunks that
%	amortizes cost. 

%One of the major differences between Redis and Memcached that heavily
%influenced the porting procedure to persistent memory was the differing
%allocation schemes. Just as a designer should aim to reduce the number of
%writes in persistent memory, they should also aim to reduce the number of
%allocations in persistent memory due to its high cost and performance
%inefficiency. Having a per-key value pair allocation schema in a volatile key
%value store is still reasonable as the performance costs of volatile
%allocation are negligible and the complexity of managing larger allocations
%can be cumbersome. However, persistent allocations require writes to
%persistent memory which incurs a much larger performance cost than volatile
%writes.  The major design choice we observed with Redis' per key value
%allocation schema and Memcached's slab-based allocation schema was that
%allocating persistent data in larger chunks greatly helps amortize the costs
%of allocation. This way, operational performance is maintained with
%allocations only being necessary when allocating a new slab.

%\end{enumerate}


==> section/impl.tex <==
\section{Implementation}


==> section/scratch_eval.tex <==
%Histograms show that Fully persistent latencies are twice as badd
%as Hybrid.
%with the Fully Persistent distributions having
%peaks and tail datapoints occurring later than in the Hybrid distributions. 


%The tail latency of Fully Persistent Redis goes up
% to around 1307 $\mu$s compared to Hybrid Redis' tail latency of 567 $\mu$s.

%Therefore, in the case of maintaining SLAs which have to ensure a certain
%throughput, choosing to utilize a Hybrid Persistent Design for its lower tail
%latency is a more reliable choice than the Fully Persistent Design.  This is
%also supported by our histograms in 
%Figures \ref{fig:redis_latency_histogram} and
%\ref{fig:memcached_latency_histogram} with the Fully Persistent distributions having
%peaks and tail datapoints occurring later than in the Hybrid distributions. In
%the Redis histograms, the Fully Persistent Distribution is bimodal with it
%second peak occuring half a magnitude higher than the Hybrid Distribution's
%peak. In the Memcached histograms the Fully Persistent Distribution's peak
%occurs a magnitude higher than the Hybird Distribution's peak.

%This is also supported by our histograms in Figures \cite{fig:Redis Histogram}
%and \cite{fig:Memcached Histogram} with the distributions being closer For
%example, from examining Figure \ref{fig:Fully Persistent Redis PDF}, you can
%see that the tail latency of Fully Persistent Redis reaches as high as 1600
%$\mu$s which is 62.5\% higher than Hybrid Redis' tail latency of around 600
%$\mu$s. Therefore, in the case of maintaining SLAs which have to ensure a
%certain throughput, choosing to utilize a Hybrid Persistent Design for its
%lower tail latency is a more reliable choice than the Fully Persistent Design.

%\todo{need YCSB results for Base Redis and Memcached as well} \rbs{These are coming????}
%\rph{missing workload F?}\rbs{F????}
%
%We also measured the throughput of Redis and Memcached on YCSB Workloads A,B,C,
%and D in order to reconfirm our conclusions using a more general dataset. From
%inspection of Figures \ref{fig:Redis_YCSBA}, \ref{fig:Redis_YCSBB},
%\ref{fig:Redis_YCSBC}, and \ref{fig:Redis_YCSBD}, Hybrid Redis remains more
%efficient than Fully Persistent Redis averaging at about 2k-5k
%operations/second faster in the four workloads. For Memcached, these trends are
%also reflected in Figures \ref{fig:Memcached_YCSBA}\ref{fig:Memcached_YCSBB},
%\ref{fig:Memcached_YCSBC}, and \ref{fig:Memcached_YCSBD} with an increase in
%throughput for Hybrid Memcached ranging anywhere from 10k to 20k
%operations/second more than Fully Persistent Memcached.

%From inspection of Figures \ref{fig:Redis_YCSBA}, \ref{fig:Redis_YCSBB},
%\ref{fig:Redis_YCSBC}, and \ref{fig:Redis_YCSBD}, Hybrid Redis remains more
%efficient than Fully Persistent Redis averaging at about \% faster in the four
%workloads. For Memcached, these trends are also reflected in Figures
%\ref{fig:Memcached_YCSBA}\ref{fig:Memcached_YCSBB}, \ref{fig:Memcached_YCSBC},
%and \ref{fig:Memcached_YCSBD} with an increase in throughput ranging from \%
%to \%.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=3.2in]{Memcached_YCSBA.png}
%   \caption{Memcached YCSB Workload A}
%   \label{fig:Memcached_YCSBA}
% \end{figure}

%From the Hybrid Redis perspective, we expected that having our data in
%persistent memory rather than in Disk would cause it to be perform better. In
%, we can see that Hybrid Redis actually performed
%slightly worse than Base Redis due to the inefficient linked list
%implementation of pmdk’s pmemobj pool allocation iterator. When measured by
%subtracting the iterator time from total time \rph{the subtraction result is meaningless
%because obviously we cannot do iteration with 0 cost. If you want to make 
%the point is their linked list implementation is inefficient, it should include
%a line with "Hybrid + optimized\_linked\_list"}, it was faster than Base Redis by
%a small constant of around 0.05 seconds \rph{use $ms$ as the unit here}.

%\rph{Should probably show performance results sections first and move recovery section afterwards}
%We begin by measuring Redis’ restart time, the length of time that Redis
%requires to accept new requests on restart. For Base Redis this involves the
%time it takes to reconstruct the hashtable by using RDB disk-based snapshot
%recovery \rph{We need to illustrate this in the figure 9 and 10 legends. It's not just base Redis but Redis with RDB enabled}. 
%Hybrid Redis has to reconstruct its hashtable and re-populate it with
%the nonvolatile data. Fully Persistent Redis is required to reconstruct its
%pointers to its persistent hashtable and data. 

%We inserted sets of unique key-value pairs into Redis with workloads
%constructed of 100k, 200k, 300k, 400k and 500k inputs. After insertion, we
%promptly shut down Redis and then measure the length of time that Redis takes
%to restart Redis according to the definitions we elaborated on.

%In Figure \ref{fig:recovery_tx}, our Fully Persistent Redis had around 10x
%worse recovery time than Base Redis and Hybrid Redis. Through some deeper
%analysis, we were able to find out that the use of transactions was causing the
%recovery to take much longer due to transactions having to persist and flush
%all persistent changes as well as log all persistent operations. In Figure
%\ref{fig:linked_list}, Fully Persistent Redis’ recovery time drops by a scale
%of over 50x after getting rid of transactions. As a result, Fully Persistent
%Redis matched our intuition of having a faster recovery time than Hybrid Redis
%but only when it got rid of transactions.

%We wished to show the increased recovery performance that the hashtable in
%persistent memory would have compared to the hashtable in volatile memory as a
%tradeoff between keeping indexing structures and data in NV memory.

% However, contrary to our opinions, in Figure \ref{fig:recovery_tx}, our Fully
% Persistent Redis had around 10x worse recovery time than Base Redis and
% Hybrid Redis. Through some deeper analysis, we were able to find out that the
% use of transactions was causing the recovery to take much longer due to
% transactions having to persist and flush all persistent changes as well as
% log all persistent operations. In Figure \ref{fig:linked_list}, Fully
% Persistent Redis’ recovery time drops by a scale of over 50x after getting
% rid of transactions. As a result, Fully Persistent Redis matched our
% intuition as it was the fastest for recovery time but only when it got rid of
% transactions. It’s possible to eliminate this by having Fully Persistent
% Redis use offsets instead of pointers, but would require significant coding
% effort from the developer and duplication of code.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\textwidth]{redis_ycsb_workload_throughput.eps}
%   \caption{Redis throughput under YCSB workload.}
%   \label{fig:redis_ycsb}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=2.7in]{memcached_ycsb_workload_throughput.eps}
%   \caption{Memcached throughput under YCSB workload.}
%   \label{fig:memcached_ycsb}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=2.7in]{redis_ycsb_client_throughput.eps}
%   \caption{Redis throughput for YCSB workloads with different number of clients.}
%   \label{fig:redis_ycsb_client_throughput}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=3.2in]{Figure_5.png}
%   \caption{Throughputs of YCSB Persistent HT Multiple Clients}
%   \label{fig:Persistent HT Mult}
% \end{figure}
% 
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=3.2in]{Figure_6.png}
%   \caption{Throughputs of YCSB Persistent Data Multiple Clients}
%   \label{fig:Persistent Data Mult}
% \end{figure}
% 
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=3.2in]{Figure_7.png}
%   \caption{Throughputs of YCSB Base Redis Multiple Clients}
%   \label{fig:Base Redis Mult}
% \end{figure}

%From a logical perspective, we expected that having a fully persistent indexing structure and
%data would decrease throughput due to the added latency that Persistent Memory
%has for writes. For all three systems, the resizing/rehashing of the hash table
%would degrade throughput. As we can see from the figure, whenever 
%The hashtable resizes after insertions reach a powers of two (16k, 32k, 64k, etc.).
%All variants show a throughput drop.  The kkkk
%
%throughput at the time of rehashing drops for each of the three systems. As a
%result, Fully Persistent Redis has the highest degradation of throughput due to
%managing a persistent indexing structure inside of transactions. 
%This shows that in cases where we have SLAs with costs to match, using Hybrid
%Redis would be a very suitable choice, as it is guarantees a very stable
%throughput, while Fully Persistent Redis and Base Redis have much larger drops
%in throughput. 
%This shows that for those who prioritize stable performance alongside
%persistence, Hybrid Redis would be a very suitable choice, as it guarantees a
%higher average throughput than Fully Persistent Redis and a more stable
%throughput during resizing than both Base Redis and Fully Persistent Redis.



==> section/stash_design.tex <==
%In this design, we chose not to place our indexing structure in nonvolatile
%memory as the complexity of Redis’ hash table would incur a large amount of
%allocations and writes to nonvolatile memory, specifically during resizing,
%thus affecting Operational Throughput. 

%This design offers reliability in terms of data, but does not exploit the
%potential of extremely fast recovery due to the costs of managing persistent
%memory. For the startup, it was required to keep track of all the persistent
%memory allocations at the time of key insertion/updations in order to properly
%recover all data. As a result, we focused our system design on optimizing
%Operational Throughput at the cost of Recovery Performance. During the
%implementation process, we encountered a variety of system design choices and
%performance issues that led us to construct two different implementations of
%Hybrid Redis, the bookKeeper version and a linked list version, each with its
%own tradeoffs. 

%\subsubsection{bookKeeper}
%Our first approach was to use a linear structure, called bookKeeper, that would keep track of all persistent memory allocations for a query.

%As we choose not to keep Redis’ original hashtable inside of persistent
%memory, the persistent data is allocated in a random order, decided by pdmk’s
%allocator, inside of libpmemobj’s memory mapped persistent file. Without a
%proper data structure to hold the allocated data upon shutdown, there is no
%way to actually access this data when restarting, effectively causing this
%data to become inaccessible memory leaks. Therefore, we created a bookKeeper
%structure as seen in Figure \ref{fig:bookKeeper}, for each key-val pair that
%Redis creates. This bookKeeper structure contains the offsets, with respect to
%the root of the persistent memory mapped file that libpmemobj creates, of all
%the allocated persistent memory relevant to a single key-value pair. The
%bookKeeper itself is stored in persistent memory contiguously, beginning 8
%bytes after the beginning of the persistent file. The first 8 bytes is where
%the number of bookKeeper entries (which directly corresponds to the number of
%key value pairs) is stored. 

%\begin{figure}[t]
%  \centering
%  \includegraphics[width=3.2in]{FAST_First.png}
%  \caption{BookKeeper Structure that stores key-value data inside of persistent memory file}
%  \label{fig:bookKeeper}
%\end{figure}

%\paragraph{Basic Queries}
%The primary purpose of the bookKeeper is to keep track of where persistent
%data lies in the file. However, since Redis is still operating on the volatile
%hashtable, the bookKeeper entries have to be modified alongside the volatile
%hashtable in real time. Persistent Memory Reads offer comparable performance
%to DRAM, but writing to Persistent Memory is comparatively slower. This
%compounded with the fact that our bookKeeper entries incur a linear lookup
%time for modifications negatively affects Operational Throughput.

%For the SET Query, there are two cases, the key does not exist or the key
%already exists.  In the event that the key does not exist, a new bookKeeper
%Entry is created and added to the end of the contiguous list. If the key
%already exists, an Update operation is required. A lookup is performed to find
%the existing bookKeeper Entry. Then, the previous value persistent data is
%freed,the newly allocated persistent offsets are added to the bookKeeper, and
%the bookKeeper count at the persistent file’s root is incremented. In both
%cases, these modifications are done alongside the updates to the volatile
%hashtable.  During DELETE Queries we similarly have to perform a lookup to
%find the bookKeeper Entry to delete and also decrement the count of
%bookKeepers at the root of the persistent file. In order to deal with
%fragmentation, the last bookKeeper entry of the contiguous list is moved into
%the spot of the recently deleted bookKeeper entry. 

%\paragraph{Restart}
%At restart, a linear pass through of the pseudo-linked list bookKeeper
%structure is made and each bookKeeper entry’s persistent data is added into
%the new, volatile hashtable. By looking at the root of the persistent file and
%getting the first bookKeeper count, we are able to figure out the number of
%bookKeepers to read from. For each offset, we added the offset to the new root
%address of the persistent memory mapped file to get new persistent pointers to
%the data. Due to the two facts that Persistent Memory has a read latency on a
%similar magnitude as main memory and we only need to read bookKeeper entries
%for reconstruction, our bookKeeper design showed slightly better Recovery
%Performance than Base Redis.  

%However, we quickly realised the design choice of a linear structure made
%updation/deletion very inefficient, as the query would require us to find the
%entry corresponding to the key, and modify it with new allocations, thus
%increasing the operational cost and the complexity of operation to O(N).

%\subsubsection{Allocator Linked List}
%In order to avoid the maintenance costs of using an auxiliary data structure, 

%allocation. The libpmemobj allocator tags these persistent memory allocations
%with the typenum and then developers are able to later iterate through
%allocated objects with specific typenums using inbuilt macros as seen in Figure
%. Using this feature, we assigned each type of allocation
%(key robjs, key sds, val robj, etc.) to different typenums so that we could
%differentiate between different allocations upon restart. 


% where we add the key robj and val robj addresses
%into the robj structure. In addition, the key robj address was added to the
%dict entry as Redis is dependent on the dict entry’s information on keys when
%performing lookups in the hashtable. We then tagged the key robj’s with a
%unique value, and at restart, looped over them to recover all the offsets
%corresponding to every key allocation/update. 

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=3.2in]{new_key_and_dict.png}
%   \caption{Modified key robj and dict entry to store persistent memory addresses for Redis Restart}
%   \label{fig:new_key}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=3.2in]{robj.png}
%   \caption{Modified key robj to store persistent memory addresses for Redis Restart}
%   \label{fig:new_key}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=3.2in]{dictEntry.png}
%   \caption{Modified dict entry to store persistent memory addresses for Redis Restart}
%   \label{fig:new_key}
% \end{figure}

%\subsubsection{Development Challenges}
%Overall, the bookKeeper design was much simpler to develop from a conceptual
%perspective and caused much fewer bugs. The main difficulties with the
%bookKeeper design was to ensure that whenever you modified the volatile
%hashtable, you had to mirror that change inside of the bookKeeper list.
%Failing to do so leads to inconsistencies in data across restart of the
%application.  The allocator linked list gives the problem of interaction
%between persistent and non-persistent structures, thus potentially
%compromising the data reliability and partial inconsistent states.  PMDK uses
%transactions to ensure data consistency in systems, therefore any persistent
%memory modifications are added to an undo log. If a transaction is aborted,
%all changes to persistent memory is rolled back, however, all of the
%modifications to volatile memory are not rolled back, leading to silent data
%inconsistencies. As a result, the onus is on the programmer to make changes to
%their code structure/flow to avoid it.

%\begin{figure}[t]
%  \centering
%  \includegraphics[width=3.2in]{bookKeeper_vs_allocated.png}
%  \caption{Throughput of bookKeeper vs allocated linked list while inserting 100,000 key-value pairs}
%  \label{fig:book vs allocated}
%\end{figure}

%\subsubsection{Comparison of two systems}
%The bookKeeper implementation was an example of a straightforward design you
%can make when porting systems to Persistent Memory. It had the added benefit
%of being simpler to implement as you have much fewer development challenges.
%In addition to the development issues listed above, in the bookKeeper design,
%you do not have to change the internal structures of Redis, leading to fewer
%indirect bugs. However, you experience (ADD STATISTICS LATER) drop in
%Operational Throughput as seen in Figure \ref{fig:book vs allocated}. The
%Allocator Linked List structure showed more improvement in Operational
%Throughput, however its design and Recovery Performance is highly dependent on
%the library you choose for persistent memory development. For example, PMDK’s
%allocator linked list does not separate typenum allocations into different
%linked lists, as seen in Figure \ref{fig:linked_list}, leading to recovery
%performance to be poorer than expected as we will discuss later in Section 6.
%If you choose a library that has an inefficient data structure or a library
%that does not keep track of allocations, you may be forced to implement your
%own data structure design similar to the bookKeeper implementation.


